Learning Locomotion Controllers for Walking Using Deep FBSDE

In this paper, we propose a deep forward-backward stochastic differential equation (FBSDE) based control algorithm for locomotion tasks. We also include state constraints in the FBSDE formulation to impose stable walking solutions or other constraints that one may want to consider (e.g., energy). Our approach utilizes a deep neural network (i.e., LSTM) to solve, in general, high-dimensional Hamilton-Jacobi-Bellman (HJB) equation resulting from the stated optimal control problem. As compared to traditional methods, our proposed method provides a higher computational efficiency in real-time; thus yielding higher frequency implementation of the closed-loop controllers. The efficacy of our approach is shown on a linear inverted pendulum model (LIPM) for walking. Even though we are deploying a simplified model of walking, the methodology is applicable to generalized and complex models for walking and other control/optimization tasks in robotic systems. Simulation studies have been provided to show the effectiveness of the proposed methodology.

==> mpc.tex <==
\section{Model Predictive Control}
The dynamics model is defined in~\eqref{eq:SDE}. If we choose a preview horizon of $N$ time steps we can have
\begin{align*}
    x_1 &= f(x(t_0), t_0)\Delta{t} + g(x(t_0), t_0)u_0\Delta{t} + \Sigma(x(t_0), t_0)\Delta{w}_0 + x_0\\
    x_2 &= f(x(t_1), t_1)\Delta{t} + g(x(t_1), t_1)u_1\Delta{t} + \Sigma(x(t_1), t_1)\Delta{w}_1 + x_1\\
        &\vdots\\
    x_N &= f(x(t_{N-1}), t_{N-1})\Delta{t} + g(x(t_{N-1}), t_{N-1})u_{N-1}\Delta{t} + \Sigma(x(t_{N-1}), t_{N-1})\Delta{w}_{N-1} + x_{N-1}
\end{align*}
where $x_0$ is the current state. This can be simplified as
\begin{equation}
    x_i = f(x(t_{i-1}), t_{i-1})\Delta{t} + g(x(t_{i-1}), t_{i-1})u_{i-1}\Delta{t} + \Sigma(x(t_{i-1}), t_{i-1})\Delta{w}_{i-1} + x_{i-1},\ i\in\{1, 2, \hdots, N\}.
\end{equation}
Let's consider a preview horizon of $N = 3$. We have the equations
\begin{align*}
    x_1 &= f(x(t_0), t_0)\Delta{t} + g(x(t_0), t_0)u_0\Delta{t} + \Sigma(x(t_0), t_0)\Delta{w}_0 + x_0\\
    x_2 &= f(x(t_1), t_1)\Delta{t} + g(x(t_1), t_1)u_1\Delta{t} + \Sigma(x(t_1), t_1)\Delta{w}_1 + x_1\\
    x_3 &= f(x(t_2), t_2)\Delta{t} + g(x(t_2), t_2)u_2\Delta{t} + \Sigma(x(t_2), t_2)\Delta{w}_2 + x_2.
\end{align*}

==> stableWalkingAlg.tex <==
\begin{algorithm}[t]
\caption{Walking Algorithm}
\begin{algorithmic}[1]
    \State {\bf Given}:
    \State $M$: number of foot steps, $N$: timesteps per foot step, $f_c(x, h, \theta)$: controller network, $H_0(x, \phi)$: initial hidden state network, $x_0$: initial state, $f$, $G$, $\Sigma$: state dynamics; $R$: Cost function parameters; $U(x)$: update rule;
    \For {$m = 1$ to $M$}
        \State $h = H_0(x, \phi)$;
        \State $x = x_0$;
        \For {$n = 1$ to $N$}
            \State $V_x, \Tilde{h} = f_c(x, h, \theta)$
            \State $u^* = -R^{-1}G^TV_x$
            \State $dx = fdt + Gu^*dt + \Sigma dw(t)$
            \State $x = x + dx$
            \State $h = \Tilde{h}$
        \EndFor
        \State Update state $x_0 = U(x)$
    \EndFor
\end{algorithmic}
\label{alg:walkingAlg}
\end{algorithm}
